Efficient Fusion and Task Guided Embedding for End-to-end Autonomous Driving

To address the challenges of sensor fusion and safety risk prediction, contemporary closed-loop autonomous driving neural networks leveraging imitation learning typically require a substantial volume of parameters and computational resources to run neural networks. Given the constrained computational capacities of onboard vehicular computers, we introduce a compact yet potent solution named EfficientFuser. This approach employs EfficientViT for visual information extraction and integrates feature maps via cross attention. Subsequently, it utilizes a decoder-only transformer for the amalgamation of multiple features. For prediction purposes, learnable vectors are embedded as tokens to probe the association between the task and sensor features through attention. Evaluated on the CARLA simulation platform, EfficientFuser demonstrates remarkable efficiency, utilizing merely 37.6% of the parameters and 8.7% of the computations compared to the state-of-the-art lightweight method with only 0.4% lower driving score, and the safety score neared that of the leading safety-enhanced method, showcasing its efficacy and potential for practical deployment in autonomous driving systems.

==> section/2-Related_works.tex <==
\section{Related Works}

\subsection{End-to-end Autonomous Driving}

    The rise of learning-based approaches has propelled end-to-end autonomous driving to the forefront of research. Two main paradigms dominate: reinforcement learning\cite{Kendall2019DriveInDay, Toromanoff2020ModelFreeRL} (RL) and imitation learning (IL). While RL holds promise for robustifying against data distribution shifts, recent advancements in driving scene generation technology\cite{shao2023reasonnet,hu2023gaia1}, coupled with the growing availability of data from new energy vehicles, have made imitation learning increasingly attractive. 

    Imitation learning approaches, particularly behavior cloning, leveraged recorded expert data to train models with high data efficiency. This data typically included two forms: trajectories and control actions. Early end-to-end AD systems utilized convolutional neural networks (CNNs) to extract image features and directly imitate control actions. However, limited by data availability and computational power, these early systems struggled to achieve good performance. Subsequently, most research shifted towards predicting trajectories instead, aiming to capture higher-level driving plans and potentially improve robustness.
 
    LBC\cite{Chen2019LBC} utilizes policy distillation where a teacher model, trained with ground-truth BEV semantic maps, predicts future waypoints. A separate student model, using only image data, then learns from the teacher's predictions. Building upon LBC, LAV\cite{Chen2022LAV} incorporates the behavior of other vehicles as intermediate supervision, potentially improving the model's robustness. TransFuser\cite{Prakash2021transfuser1,Chitta2023transfuser2}, utilizes two CNNs to extract image and LiDAR information, followed by a transformer to fuse this information at each downsampling step, potentially capturing richer contextual cues. Similarly, InterFuser\cite{shao2022interfuser} extracts sensor features with CNNs, but leverages an encoder-decoder structure to additionally incorporate traffic rules and vehicle density information, aiming for more comprehensive decision-making through this enhanced understanding of the driving environment.

    In terms of behavior cloning, CIL\cite{Codevilla2019CIL} selectively learns control actions and introduces additional intermediate supervision. TCP\cite{Wu2022TCP} introduces control actions within a sequence of time into training, and uses a control method that mixes trajectory (i.e. waypoints) trackers and behavior prediction results. Both approaches achieve impressive results with single-view images, making them suitable for resource-constrained hardware and paving the way for real-world applications.

\subsection{Efficient Deep Neural Network}

    Deep neural networks have revolutionized various fields, but their hefty computational demands often restrict their deployment on resource-constrained platforms. To address this challenge, researchers have developed a diverse arsenal of efficient network architectures and techniques. MobileNets\cite{sandler2019mobilenetv2,howard2019mobilenetv3}, for example, utilize clever architectural choices like depthwise separable convolutions to achieve significant computational savings without sacrificing accuracy. MCUNet\cite{lin2020mcunet,lin2021mcunetV2} represents the epitome of miniaturization, squeezing networks onto embedded platforms with a mere 256KB of memory, opening doors for AI deployment previously unimaginable. NetAug\cite{Han2022netaug} tackles the challenge from a different angle, training tiny networks within larger ones as "inner teachers" to provide crucial supervision for efficient learning. ShiftAddAug\cite{guo2024shiftaddaug} goes step further and introduce this method to multiplication-free networks for better hardware-efficiency.


    
